Incorporating non-local anyonic statistics into a graph decomposition

In this work we describe how to systematically implement a full graph decomposition to set up a linked-cluster expansion for the topological phase of Kitaev's toric code in a field. This demands to include the non-local effects mediated by the mutual anyonic statistics of elementary charge and flux excitations. Technically, we describe how to consistently integrate such non-local effects into a hypergraph decomposition for single excitations. The approach is demonstrated for the ground-state energy and the elementary excitation energies of charges and fluxes in the perturbed topological phase.

==> Preamble.tex <==
\usepackage{tikz}
\usepackage{braket}
\usepackage{xcolor}
%FAUcolors
\definecolor{FAUblau}{RGB}{4,49,106}
\definecolor{FAUdunkelblau}{RGB}{4,30,66}
\definecolor{FAUgelb}{RGB}{253,183,53}
\definecolor{FAUorange}{RGB}{232,119,34}
\definecolor{FAUrot}{RGB}{197,15,60}
\definecolor{FAUdunkelrot}{RGB}{151,27,47}
\definecolor{FAUmedblau}{RGB}{24,180,241}
\definecolor{FAUmeddunkelblau}{RGB}{0,82,135}
\definecolor{FAUgruen}{RGB}{123,183,37}
\definecolor{FAUdunkelgruen}{RGB}{38,97,65}
\definecolor{FAUmetallic}{RGB}{140,159,177}
\definecolor{FAUdunkelmetallic}{RGB}{47,88,110}
%mmcommands
\DeclareRobustCommand{\tcplaq}
{
	{\hbox{\begin{tikzpicture}[x=1 ex, y = 1 ex, scale = 0.25, style={inner sep=0,outer sep=0}, line cap = round, line join= round, line width = 0.8]
			\draw  (0,0) rectangle(3 ,3);
			\end{tikzpicture}}
	}
}

\DeclareRobustCommand{\tcstar}
{
	{
		\hbox{\begin{tikzpicture}[x=1 ex, y = 1 ex, scale = 0.25, style={inner sep=0,outer sep=0},line cap = round, line join= round, line width = 0.8]
			\draw  (0,1.5) -- (3,1.5) ;
			\draw  (1.5,0) -- (1.5,3) ;
			\end{tikzpicture}}
	}
}
\DeclareRobustCommand{\bigtcplaq}
{
	{\hbox{\begin{tikzpicture}[x=1 ex, y = 1 ex, scale = .35, style={inner sep=0,outer sep=0}, line cap = round, line join= round, line width = 1]
			\draw  (0,0) rectangle(3 ,3);
			\end{tikzpicture}}
	}
}

\DeclareRobustCommand{\bigtcstar}
{
	{
		\hbox{\begin{tikzpicture}[x=1 ex, y = 1 ex, scale = .35, style={inner sep=0,outer sep=0},line cap = round, line join= round, line width = 1]
			\draw  (0,1.5) -- (3,1.5) ;
			\draw  (1.5,0) -- (1.5,3) ;
			\end{tikzpicture}}
	}
}

